What makes fake images detectable? Understanding properties that generalize

The quality of image generation and manipulation is reaching impressive levels, making it increasingly difficult for a human to distinguish between what is real and what is fake. However, deep networks can still pick up on the subtle artifacts in these doctored images. We seek to understand what properties of fake images make them detectable and identify what generalizes across different model architectures, datasets, and variations in training. We use a patch-based classifier with limited receptive fields to visualize which regions of fake images are more easily detectable. We further show a technique to exaggerate these detectable properties and demonstrate that, even when the image generator is adversarially finetuned against a fake image classifier, it is still imperfect and leaves detectable artifacts in certain image patches. Code is available at https://chail.github.io/patch-forensics/.

==> sec_acknowledgements.tex <==
\paragraph{Acknowledgements.} We would like to thank Antonio Torralba, Jonas Wulff, Jacob Huh, Harry Yang, and Richard Zhang for helpful discussions. This work was supported by a National Science Foundation Graduate Research Fellowship under Grant No. 1122374 to L.C. and DARPA XAI FA8750-18-C000-4 to D.B.

==> sec_method.tex <==
\section{Using Patches for Image Forensics}

Rather than training a network to predict a global ``real'' or ``fake'' decisions for an image, we use shallow networks with limited receptive fields that focus on small patches of the image. This approach allows us to localize regions of the image that are detected to be manipulated and ensemble the patch-wise decisions to obtain the overall prediction.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\textwidth]{figures/01_schematic.pdf} % , trim=0 700 0 0, clip
% \vspace{-0.3in}
\caption{We use a classifier with small receptive fields to obtain a heatmap over the patch-wise output. To obtain this patch classifier, we truncate various deep learning models after an initial sequence of layers.}
\label{fig:schematic}
\vspace{-0.1in}
\end{figure}

\subsection{Models for patch-based classification.}

Modern deep learning architectures typically consist of a series of modular blocks. By truncating the models after an intermediate block, we can obtain model predictions based on a local region of the image, where truncating earlier in the layer sequence results in a smaller receptive field, while truncating after more layers results in a larger receptive field. We then add a 1x1 convolution layer after this truncated backbone to convert the feature representation into a binary real-or-fake prediction. We experiment with Resnet and Xception as our model backbones -- generally we observe that Xception blocks perform better than Resnet blocks, however we also report results of the top performing Resnet block. We provide additional details on the model architecture and receptive field calculations in Supplementary Material Sec.~\ref{apx:architecture}.

The truncation operation reduces the size of the model's receptive field, and yields a prediction for a receptive-field-sized patch of the input, rather than the entire image at once. This forces the models to learn local properties that distinguish between real and fake images, where the same model weights are applied in a sliding fashion over the entire image, and each output prediction is only a function of a small localized patch of the image. We apply a cross entropy loss to each patch; i.e. every real patch should be considered real, and every fake image patch should be considered fake:
\begin{equation}
    \mathcal{L}(\mathbf{x}) = \frac{1}{|P|}\sum_{i,j}\sum_t t\log f^t(x_{i,j})
\end{equation}
where $f$ is the model output after a softmax operation to normalize the logits, $t$ indexes over the real and fake output for binary classification, $(i,j)$ indexes over the receptive field patches, and $|P|$ is the total number of patches per image. We train these models with the Adam optimizer with default learning rate, and terminate training when validation accuracy does not improve for a predetermined number of epochs.

By learning to classify patches, we increase the ratio of data points to model parameters: each patch of the image is treated independently, and the truncated models are smaller. The final classification output is an ensemble of the individual patch decisions rather than a single output probability. To aggregate patches at inference time, we take a simple average after applying a softmax operation to the patch-wise predictions: 
\begin{equation}
    t^* = \arg\max_t  \left(\frac{1}{|P|}\sum_{i,j} f^t(x_{i,j})\right)
\end{equation}
The averaging approach can be applied in both cases where the image is wholly generated, or when only part of the image is manipulated. For example, when a generated face is spliced onto a real background, the background patches may not be predicted as fake; in this case, because the same background is present in both real and fake examples, the model remains uncertain in these locations.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\textwidth]{figures/02_preprocessing.pdf} % , trim=0 510 0 0, clip
% \vspace{-0.3in}
\caption{To minimize the effect of image preprocessing artifacts - in which real and fake images undergo different preprocessing operations -- we pass real images through the same data transform as used to train the generator. We then save the real and fake images using identical pipelines.}
\label{fig:preprocessing}
\vspace{-0.1in}
\end{figure}

\subsection{Dataset preparation} 

\subsubsection{Image preprocessing.} A challenge with fully generative images, such as those created by GANs, is that fake images can be saved with arbitrary codecs, e.g., we decide whether we want to save the image in JPG or PNG format. However, the set of real images is saved with a fixed codec when the original dataset is created. When training a classifier on real and fake images with subtly different preprocessing pipelines, the classifier can simply learn to detect the differences in preprocessing. If the test images also have this inconsistency, we would appear to obtain high accuracy on the test set, even though the classifier is really only detecting formatting artifacts. One way to mitigate this disparity is to apply data augmentation to reduce the effect of these differences~\cite{wang2019cnn,xuan2019generalization}.

We preprocess the images to make our real and fake dataset as similar as possible, in an effort to isolate fake image artifacts and minimize the possibility of learning differences in preprocessing. We create the ``real'' dataset by passing the real images through the generator's data loading pipeline (e.g. resizing) and saving the real images \textit{after} this step in lossless PNG format (Fig.~\ref{fig:preprocessing}). We save the fake images in PNG format from the generator output, so the remaining differences between real and fake images are due to artifacts of the generator. We then resize all images to the same size using Lanczos interpolation before saving to file. Additional details are provided in Supplementary Material Sec.~\ref{apx:preprocessing}.

We take these precautions because any minor difference in preprocessing is easily learnt by the fake-image classifier and leads to an illusion of increased generalization capacity (for example, differences in the image codec leads to perfect average precision across various test datasets; see Supplementary Material Sec.~\ref{apx:preprocessing}). This approach allows us to focus on the inherent differences between real images and generated ones to minimize any potential confounders due to preprocessing. In the remainder of this section, we briefly detail the image generation and manipulation methods that we investigate in our experiments.

\vspace{-0.1in}
\subsubsection{Fully Generative Models.} The first class of models we consider are fully generative models which map a random sample from a known distribution (e.g. a multivariate Gaussian) to an image. \textit{Progressive GAN} (PGAN)~\cite{karras2017progressive} is one recent example, which uses a progressive training schedule to increase the output resolution of images during training. We use the publicly available PGAN model trained on the CelebA-HQ face dataset. We also train several other PGANs to various smaller resolutions and on the more diverse FFHQ face dataset. \textit{StyleGAN} (SGAN)~\cite{karras2019style} introduces an alternative generator architecture which incorporates the latent code into intermediate layers of the generator, resulting in unsupervised disentanglement of high-level attributes, e.g., hair and skin tone.
We use the public versions of StyleGAN on the CelebA-HQ and FFHQ datasets, and StyleGAN2 \cite{karras2019analyzing} on the FFHQ dataset. In additional to PGAN and SGAN, we also consider the \textit{Glow} generator~\cite{kingma2018glow}, a flow-based model using modified 1x1 invertible convolutions that optimizes directly for log-likelihood rather than adversarial loss. We use the public Glow generator trained on CelebA-HQ faces. Finally, we also include a face generator based on a \textit{Gaussian Mixture Model} (GMM) rather than convolutional layers~\cite{richardson2018gans}; the GMM uses low-rank plus diagonal Gaussians to efficiently model covariance in high-dimensional outputs such as images. We train the GMM model on the CelebA~\cite{liu2015faceattributes} dataset using default parameters.

\subsubsection{Facial Manipulation Models.} We use the FaceForensics++ dataset~\cite{rossler2019faceforensics++}, which includes methods for identity manipulation and expression transfer. Identity manipulation approaches, such as \textit{FaceSwap}, paste a source face onto a target background; specifically, FaceSwap fits detected facial landmarks to 3D model and then projects the face onto the target scene. The deep learning analogue to FaceSwap is the \textit{Deepfake} technique, which uses a pair of autoencoders with a shared encoder to swap the source and target faces. On the other hand, expression transfer maps the expression of a source actor onto the face of a target. \textit{Face2Face} achieves this by tracking expression parameters of the face in a source video and applying them to a target sequence. \textit{Neural Textures} uses deep networks to learn a texture map and a neural renderer to modify the expression of the target face. 
\subsection{Baseline Models.}

We train and evaluate full MesoInception4~\cite{afchar2018mesonet}, Resnet~\cite{he2016deep}, and Xception~\cite{chollet2017xception} models on the same datasets that we use to train the truncated classifiers. Following~\cite{afchar2018mesonet}, we train MesoInception4 using squared error loss. For the Resnet model and the Xception model, also used in~\cite{rossler2019faceforensics++}, we train with standard two-class cross entropy loss. We train these models from scratch as they are not initially trained for this classification task. Finally, we also compare to a model trained to detect CNN artifacts via blurring and compression augmentations~\cite{wang2019cnn}. For this model, we finetune at a learning rate of 1e-6 using similar augmentation parameters as the original paper to improve its performance specifically on face datasets. We use the same stopping criteria based on validation accuracy for all baseline models as we use for the truncated models.


